Scalable Analysis for Large Social Networks: the data-aware mean-field approach

Studies on social networks have proved that endogenous and exogenous factors influence dynamics. Two streams of modeling exist on explaining the dynamics of social networks: 1) models predicting links through network properties, and 2) models considering the effects of social attributes. In this interdisciplinary study we work to overcome a number of computational limitations within these current models. We employ a mean-field model which allows for the construction of a population-specific socially informed model for predicting links from both network and social properties in large social networks. The model is tested on a population of conference coauthorship behavior, considering a number of parameters from available Web data. We address how large social networks can be modeled preserving both network and social parameters. We prove that the mean-field model, using a data-aware approach, allows us to overcome computational burdens and thus scalability issues in modeling large social networks in terms of both network and social parameters. Additionally, we confirm that large social networks evolve through both network and social-selection decisions; asserting that the dynamics of networks cannot singly be studied from a single perspective but must consider effects of social parameters.

==> graph/epstopdf <==
#!/usr/bin/perl
use strict;

# Change by Thomas Esser, Sept. 1998: The above lines allows us to find
# perl along $PATH rather than guessing a fixed location. The above
# construction should work with most shells.

# A script to transform an EPS file so that:
#   a) it is guarenteed to start at the 0,0 coordinate
#   b) it sets a page size exactly corresponding to the BoundingBox
# This means that when Ghostscript renders it, the result needs no
# cropping, and the PDF MediaBox is correct.
#   c) the result is piped to Ghostscript and a PDF version written
#
# It needs a Level 2 PS interpreter.
# If the bounding box is not right, of course, you have problems...
#
# The only thing I have not allowed for is the case of
# "%%BoundingBox: (atend)", which is more complicated.
#
# Sebastian Rahtz, for Elsevier Science
#
# now with extra tricks from Hans Hagen's texutil.
#
# History
#  1999/05/06 v2.5 (Heiko Oberdiek)
#    * New options: --hires, --exact, --filter, --help.
#    * Many cosmetics: title, usage, ...
#    * New code for debug, warning, error
#    * Detecting of cygwin perl
#    * Scanning for %%{Hires,Exact,}BoundingBox.
#    * Scanning only the header in order not to get a wrong
#      BoundingBox of an included file.
#    * (atend) supported.
#    * uses strict; (earlier error detecting).
#    * changed first comment from '%!PS' to '%!';
#    * corrected (atend) pattern: '\s*\(atend\)'
#    * using of $bbxpat in all BoundingBox cases,
#      correct the first white space to '...Box:\s*$bb...'
#    * corrected first line (one line instead of two before 'if 0;';
#  2000/11/05 v2.6 (Heiko Oberdiek)
#    * %%HiresBoundingBox corrected to %%HiResBoundingBox
#  2001/03/05 v2.7 (Heiko Oberdiek)
#    * Newline before grestore for the case that there is no
#      whitespace at the end of the eps file.
#  2002/02/18 v2.8draft (Gerben Wierda)
#    * Handle different eol styles transparantly
#    * Applied fix from Peder Axensten for Freehand bug
#  2002/02/21 v2.8draft (Gerben Wierda)
#    * Fixed bug where last line of buffer was not copied out (ugh!)
#  2003/04/22 v2.9draft (Gerben Wierda)
#    * Fixed bug where with cr-eol files everything up to the first %!
#    * in the first 2048 bytes was gobbled (double ugh!)
#  2004/03/17 v2.9.1draft (Gerben Wierda)
#    * No autorotate page
#  2005/09/29 v2.9.2draft (Gerben Wierda)
#    * Quote OutFilename
#  2005/10/01 v2.9.3draft (Gerben Wierda)
#    * Quote OutFilename
#  2005/10/06 v2.9.4gw (Gerben Wierda)
#    * This has become the official version for now
#  2005/10/06 v2.9.5gw (Gerben Wierda)
#    * Fixed a horrendous bug in the (atend) handling code
#

### program identification
my $program = "epstopdf";
my $filedate="2006/01/29";
my $fileversion="2.9.5gw";
my $copyright = "Copyright 1998-2006 by Sebastian Rahtz et al.";
my $title = "\U$program\E $fileversion, $filedate - $copyright\n";

### ghostscript command name
my $GS = "gs";
$GS = "gswin32c" if $^O eq 'MSWin32';
$GS = "gswin32c" if $^O =~ /cygwin/;

### options
$::opt_help=0;
$::opt_debug=1;
$::opt_compress=1;
$::opt_gs=1;
$::opt_hires=0;
$::opt_exact=0;
$::opt_filter=0;
$::opt_outfile="";

### usage
my @bool = ("false", "true");
my $usage = <<"END_OF_USAGE";
${title}Syntax:  $program [options] <eps file>
Options:
  --help:           print usage
  --outfile=<file>: write result to <file>
  --(no)filter:     read standard input   (default: $bool[$::opt_filter])
  --(no)gs:         run ghostscript       (default: $bool[$::opt_gs])
  --(no)compress:   use compression       (default: $bool[$::opt_compress])
  --(no)hires:      scan HiResBoundingBox (default: $bool[$::opt_hires])
  --(no)exact:      scan ExactBoundingBox (default: $bool[$::opt_exact])
  --(no)debug:      debug informations    (default: $bool[$::opt_debug])
Examples for producing 'test.pdf':
  * $program test.eps
  * produce postscript | $program --filter >test.pdf
  * produce postscript | $program -f -d -o=test.pdf
Example: look for HiResBoundingBox and produce corrected PostScript:
  * $program -d --nogs -hires test.ps>testcorr.ps
END_OF_USAGE

### process options
use Getopt::Long;
GetOptions (
  "help!",
  "debug!",
  "filter!",
  "compress!",
  "gs!",
  "hires!",
  "exact!",
  "outfile=s",
) or die $usage;

### help functions
sub debug {
  print STDERR "* @_\n" if $::opt_debug;
}
sub warning {
  print STDERR "==> Warning: @_!\n";
}
sub error {
  die "$title!!! Error: @_!\n";
}
sub errorUsage {
  die "$usage\n!!! Error: @_!\n";
}

### option help
die $usage if $::opt_help;

### get input filename
my $InputFilename = "";
if ($::opt_filter) {
  @ARGV == 0 or
    die errorUsage "Input file cannot be used with filter option";
  $InputFilename = "-";
  debug "Input file: standard input";
}
else {
  @ARGV > 0 or die errorUsage "Input filename missing";
  @ARGV < 2 or die errorUsage "Unknown option or too many input files";
  $InputFilename = $ARGV[0];
  -f $InputFilename or error "'$InputFilename' does not exist";
  debug "Input filename:", $InputFilename;
}

### option compress
my $GSOPTS = "";
$GSOPTS = "-dUseFlateCompression=false " unless $::opt_compress;

### option BoundingBox types
my $BBName = "%%BoundingBox:";
!($::opt_hires and $::opt_exact) or
  error "Options --hires and --exact cannot be used together";
$BBName = "%%HiResBoundingBox:" if $::opt_hires;
$BBName = "%%ExactBoundingBox:" if $::opt_exact;
debug "BoundingBox comment:", $BBName;

### option outfile
my $OutputFilename = $::opt_outfile;
if ($OutputFilename eq "") {
  if ($::opt_gs) {
    $OutputFilename = $InputFilename;
    if (!$::opt_filter) {
      $OutputFilename =~ s/\.[^\.]*$//;
      $OutputFilename .= ".pdf";
    }
  }
  else {
    $OutputFilename = "-"; # standard output
  }
}
if ($::opt_filter) {
  debug "Output file: standard output";
}
else {
  debug "Output filename:", $OutputFilename;
}

### option gs
if ($::opt_gs) {
  debug "Ghostscript command:", $GS;
  debug "Compression:", ($::opt_compress) ? "on" : "off";
}

### open input file
open(IN,"<$InputFilename") or error "Cannot open",
  ($::opt_filter) ? "standard input" : "'$InputFilename'";
binmode IN;

### open output file
if ($::opt_gs) {
  my $pipe = "$GS -q -sDEVICE=pdfwrite $GSOPTS -dAutoRotatePages=/None" .
          " -sOutputFile='$OutputFilename' - -c quit";
  debug "Ghostscript pipe:", $pipe;
  open(OUT,"|$pipe") or error "Cannot open Ghostscript for piped input";
}
else {
  open(OUT,">$OutputFilename") or error "Cannot write '$OutputFilename";
}

# reading a cr-eol file on a lf-eol system makes it impossible to parse
# the header and besides it will read the intire file into yor line by line
# scalar. this is also true the other way around.

### scan a block, try to determine eol style

my $buf;
my $buflen;
my @bufarray;
my @parsedbufarray; # for mytell/myseek
my $bufarraypos;

# We assume 2048 is big enough.
my $EOLSCANBUFSIZE = 2048;

$buflen = read( IN, $buf, $EOLSCANBUFSIZE);
if ($buflen > 0) {
  my $crlfpos;
  my $lfpos;
  my $crpos;

  # remove binary junk before header
  # if there is no header, we assume the file starts with ascii style and
  # we look for a eol style anyway, to prevent possible loading of the
  # entire file
  if ($buf =~ /%!/) {
    # throw away binary junk before %!
    $buf =~ s/(.*?)%!/%!/o;
  }
  $lfpos = index( $buf, "\n");
  $crpos = index( $buf, "\r");
  $crlfpos = index( $buf, "\r\n");

  if ($crpos > 0 and ($lfpos == -1 or $lfpos > $crpos+1)) {
    # The first eol was a cr and it was not immediately followed by a lf
    $/ = "\r";
    debug "The first eol character was a CR ($crpos) and not immediately followed by a LF ($lfpos)";
  }

  # Now we have set the correct eol-character. Get one more line and add
  # it to our buffer. This will make the buffer contain an entire line
  # at the end. Then split the buffer in an array. We will draw lines from
  # that array until it is empty, then move again back to <IN>
  $buf .= <IN> unless eof( IN);
  $buflen = length( $buf);
  $bufarraypos = 0;

  # Some extra magic is needed here: if we set $/ to \r, Perl's re engine
  # still thinks eol is \n in regular expressions (not very nice) so we
  # cannot split on ^, but have to split on \r and reappend those.
  if ($/ eq "\r") {
    @bufarray = split( /\r/ms, $buf); # split on \r
    grep( $_ .= "\r", @bufarray); # re-append \r to each array item
  }
  else {
    @bufarray = split( /^/ms, $buf);
  }
}

### getline
sub getline {
  if ($#bufarray >= 0) {
    $_ = shift( @bufarray);
    unshift( @parsedbufarray, $_); # for myseek and mytell
    $bufarraypos += length( $_);
    # debug "getline from array. bufarraypos = $bufarraypos";
    # debug "*** READ: $_";
  }
  else {
    $_ = <IN>;
  }
  return( defined( $_));
}

### mytell and myseek, work on <IN> only
sub mytell {
  if ($#bufarray) {
    # debug "Telling ARRAY position $bufarraypos";
    return $bufarraypos;
  }
  else {
    my $pos = tell( IN);
    # debug "Telling FILE position $pos";
    return $pos;
  }
}

sub myseek {
  my $pos = shift;
  # debug "Seeking to position $pos in input";
  if ($pos < $buflen) {
    # debug "myseek position $pos < buffer size $buflen";
    # We were still parsing the array, reset to the end of buf and
    # move to the right line in the array.
    # Now, move stuff from the @parsedbufarray back until we are back at $pos
    my $tmpline;
    while ($bufarraypos > $pos) {
      # debug "myseek bufarray position $bufarraypos > position $pos";
      # we test on parsedbufarray to prevent an infinite loop on
      # a programming error (DEVELOP only)
      die "Programming error 1\n" unless $#parsedbufarray;
      $tmpline = shift( @parsedbufarray);
      $bufarraypos -= length( $tmpline);
      unshift( @bufarray, $tmpline);
      debug "*** UNREAD: $tmpline";
    }
    # debug "Returning to ARRAY size position $buflen (bufarraypos = $bufarraypos)";
    return seek( IN, $buflen, 0);
  }
  else {
    # debug "Seeking to FILE position $pos";
    return seek( IN, $pos, 0);
  }
}

### scan first line
my $header = 0;
getline();
if (/%!/) {
  # throw away binary junk before %!
  s/(.*)%!/%!/o;
}
$header = 1 if /^%/;
debug "Scanning header for BoundingBox";
print OUT;

### variables and pattern for BoundingBox search
my $bbxpatt = '[0-9eE\.\-]';
               # protect backslashes: "\\" gets '\'
my $BBValues = "\\s*($bbxpatt+)\\s+($bbxpatt+)\\s+($bbxpatt+)\\s+($bbxpatt+)";
my $BBCorrected = 0;

sub CorrectBoundingBox {
  my ($llx, $lly, $urx, $ury) = @_;
  debug "Old BoundingBox:", $llx, $lly, $urx, $ury;

  # Joerg's FIX: make bounding box bigger
  $llx = $llx-1;
  $lly = $lly-1;
  $urx = $urx+1;
  $ury = $ury+1;
  my ($width, $height) = ($urx - $llx, $ury - $lly);
  my ($xoffset, $yoffset) = (-$llx, -$lly);
  debug "New BoundingBox: 0 0", $width, $height;
  debug "Offset:", $xoffset, $yoffset;

  print OUT "%%BoundingBox: 0 0 $width $height\n";
  print OUT "<< /PageSize [$width $height] >> setpagedevice\n";
  print OUT "gsave $xoffset $yoffset translate\n";
}

### scan header
if ($header) {
  HEADER: while (getline()) {
    ### Fix for freehand bug ### by Peder Axensten
    next HEADER if(!/\S/);

    ### end of header
    if (!/^%/ or /^%%EndComments/) {
      print OUT;
      last;
    }

    ### BoundingBox with values
    if (/^$BBName$BBValues/) {
      CorrectBoundingBox $1, $2, $3, $4;
      $BBCorrected = 1;
      last;
    }

    ### BoundingBox with (atend)
    if (/^$BBName\s*\(atend\)/) {
      debug $BBName, "(atend)";
      if ($::opt_filter) {
        warning "Cannot look for BoundingBox in the trailer",
                "with option --filter";
        last;
      }
      my $pos = mytell();
      debug "Current file position:", $pos;

      # looking for %%BoundingBox
      while (getline()) {
        # skip over included documents
        if (/^%%BeginDocument/) {
          while (getline()) {
            last if /^%%EndDocument/;
          }
        }
        if (/^$BBName$BBValues/) {
          CorrectBoundingBox $1, $2, $3, $4;
          $BBCorrected = 1;
          last;
        }
      }

      # go back
      myseek( $pos) or error "Cannot go back to line '$BBName (atend)'";
      last;
    }

    # print header line
    print OUT;
  }
}

### print rest of file
while (getline()) {
  print OUT;
}

### close files
close(IN);
print OUT "\ngrestore\n" if $BBCorrected;
close(OUT);
warning "BoundingBox not found" unless $BBCorrected;
debug "Ready.";
;

